LHCb Detector Performance

The LHCb detector is a forward spectrometer at the Large Hadron Collider (LHC) at CERN. The experiment is designed for precision measurements of CP violation and rare decays of beauty and charm hadrons. In this paper the performance of the various LHCb sub-detectors and the trigger system are described, using data taken from 2010 to 2012. It is shown that the design criteria of the experiment have been met. The excellent performance of the detector has allowed the LHCb collaboration to publish a wide range of physics results, demonstrating LHCb's unique role, both as a heavy flavour experiment and as a general purpose detector in the forward region.

==> CALO-systeme.tex <==
\subsection{Calibration of the calorimeter system}

Each of the four parts of the calorimeter system follows a different calibration procedure. The SPD calibration is performed by adjusting the discriminator thresholds for each channel slightly below the value corresponding to the expected energy deposit of a MIP. To validate these values the efficiency is determined as the fraction of times a track pointing to a cell corresponds to a hit~\cite{CALOR-SPD}. For the PS, the response of the ADC of each channel is equalized according to the most probable energy deposition of MIP's. The MIP sample is composed of reconstructed tracks of charged particles in the LHCb tracking system, requiring their momentum to be larger 
than 2~\gevc in order to reach the PS~\cite{CALOR-PS}. 

To optimize the calibration of the ECAL a three steps process is performed. 
In the first step, the settings of each channel are fixed combining the system design values with
laboratory and test beam measurements to reproduce the design energy range. This initial calibration, used during the first LHC collisions, leads
to a $\pi^0\to\gamma\gamma$ mass resolution at the level of 10\%.
In the second step, the gains of the channels are equalised. This is achieved by applying an energy flow method based on the continuity of the
cumulative energy deposit~\cite{LHCb-DP-2013-004}. 
The third step improves the calibration coefficients by performing fits to the invariant mass
distribution of $\piz\to\gamma\gamma$ decays~\cite{CHEP-XCAL}. For this, neutral clusters consistent with single
photon signals with a small energy deposit in the PS are
considered. Only low multiplicity events are selected in order to reduce the combinatorial background and the contamination by
the underlying event. For each \piz{} candidate, the reconstructed \piz{} mass is assigned to the two cells with the highest energy deposit in each photon cluster. When enough candidates are collected, the \piz{} mass
distribution is fitted for each cell, and the energy scale of the cell
is corrected by setting the mean of the signal peak to the PDG value of the \piz{} mass.
This procedure is repeated until the obtained calibration is stable. As illustrated in Figure~\ref{fig:pi0mass}, this final calibration
step considerably improves the $\piz\to\gamma\gamma$ invariant mass
resolution. 

By applying the method to a sample of miscalibrated
simulated events, the final precision of the cell to cell intercalibration is estimated
to be approximately 2\%. The performance of the ECAL is monitored by
studying the energy to momentum ratio (\eOverP) distributions from samples of pure electrons
selected from conversions.

%Finally, the fine calibration approach uses a fitting iterative method of the \piz mass distribution from two photon combinations~\cite{CHEP-XCAL}.
%In this procedure, photons are defined from $3\times 3$ neutral clusters consistent with single photon signals, in which the cell with the highest energy
%deposit is called the seed. A selection is imposed to use only photon leaving a small energy deposit in the PS.
%The selected \piz candidates must belong to low multiplicity events in order to limit pile-up effects.
%For each cell, the di-photon invariant mass is fit. When enough statistics is reached, the energy of each seed is corrected to match the
%\piz nominal mass and the procedure is repeated until the obtained calibration is stable.
%On Figure~\ref{fig:pi0mass}, the effect of the fine calibration algorithm is reported.
%The estimated precision of the calibration reached by this method is of the order of 2\%,
%estimated by applying the method on a miscalibrated simulated sample.
%In addition, some pure electron samples selected from conversions are used to monitor ECAL performance
%by studying the energy to momentum ratio (\eOverP) distributions.

\begin{figure}[!tb]
\begin{center}
\includegraphics[width=0.6\textwidth]{../figs/calo/pi0masscal.pdf}
\end{center}
\caption{\label{fig:pi0mass} Invariant mass distribution for $\piz\to\gamma\gamma$ candidates upon which the fine calibration algorithm is applied. The red curve corresponds to the distribution before applying the method, while the blue curve is the final one. Values in the red (blue) box are the mean and sigma of the signal peak distribution before (after) applying the fine calibration method.}
\end{figure}

The calibration of the HCAL relies on two $^{137}{\rm Cs}$ sources of $\sim 10$~{mCi} each, one per detector side, which are moved through all scintillator tiles using a hydraulic system. The PMT response is measured with a dedicated system of current
integrators. The relation between the anode current and the measured particle energy is known
from test beam studies, which showed also that this method facilitates a cell-to-cell intercalibration at the
level of 5\%~\cite{LHCb-DP-2013-004}. The performance of the HCAL is monitored during the data taking periods using the built-in LED system. The channel response to the LED flashes is highly correlated with the results obtained from the $^{137}{\rm Cs}$ sources and can be used to establish new values of the correlation coefficients when the standard calibration procedure cannot be applied~\cite{LHCb-DP-2013-004}.
The final calibration of the absolute scale is performed by matching
the \eOverP distribution of well-identified hadrons to that obtained in
simulated events. 

Figure~\ref{fig:calibcoeffs} shows the ratio between the coefficients obtained from average values of \eOverP calibration method and the ones from the $^{137}{\rm Cs}$ source calibration. The results from the two methods are in agreement. Moreover, this approach allows to spot channels whose PMT shows stability issues.

\begin{figure}[!tb]
\begin{center}
\includegraphics[width=0.6\textwidth]{../figs/calo/ep_calibcoeff.pdf}
\caption{Ratio between the calibration coefficients obtained from the final \eOverP calibration and the $^{137}$Cs calibration for all HCAL channels.}
\label{fig:calibcoeffs}
\end{center}
\end{figure}
%In addition to the use of the LED system, the more precise HCAL calibration is performed on a regular basis using
%the embedded cesium radioactive source.

%A full account on the different calibration and monitoring procedures can be found in~\cite{LHCb-DP-2013-004}
%and references therein.

While no significant degradation of the SPD and the PS performances has been
seen, first signs of detector ageing have been observed in both the ECAL
and the HCAL~\cite{LHCb-DP-2013-004}. The main cause for the loss of performance is the decrease of the PMT gains. This comes from the degradation of the PMT dynode system at high integrated anode current to which some PMTs are subjected. In the case of the HCAL, the detector response has been monitored using the LED system. This allows the channel gain losses to be established and be regularly compensated by increasing the PMT high voltages. In the case of the  ECAL, the gain loss was monitored using the \eOverP ratio for electrons and also compensated by increasing the PMT high voltages.



